Skeleton-Guided-Translation: A Benchmarking Framework for Code Repository Translation with Fine-Grained Quality Evaluation

The advancement of large language models has intensified the need to modernize enterprise applications and migrate legacy systems to secure, versatile languages. However, existing code translation benchmarks primarily focus on individual functions, overlooking the complexities involved in translating entire repositories, such as maintaining inter-module coherence and managing dependencies. While some recent repository-level translation benchmarks attempt to address these challenges, they still face limitations, including poor maintainability and overly coarse evaluation granularity, which make them less developer-friendly. We introduce Skeleton-Guided-Translation, a framework for repository-level Java to C# code translation with fine-grained quality evaluation. It uses a two-step process: first translating the repository's structural "skeletons", then translating the full repository guided by these skeletons. Building on this, we present TRANSREPO-BENCH, a benchmark of high quality open-source Java repositories and their corresponding C# skeletons, including matching unit tests and build configurations. Our unit tests are fixed and can be applied across multiple or incremental translations without manual adjustments, enhancing automation and scalability in evaluations. Additionally, we develop fine-grained evaluation metrics that assess translation quality at the individual test case level, addressing traditional binary metrics' inability to distinguish when build failures cause all tests to fail. Evaluations using TRANSREPO-BENCH highlight key challenges and advance more accurate repository level code translation.

==> figures/Performance01.tex <==
\begin{table*}[htb]
    \caption{Overall Performance Evaluation of Large Language Models}
    % \begin{threeparttable}
    \small
    \centering
\begin{tabular}{lcccccc}
\toprule
\textbf{Model} & \multicolumn{2}{c}{\textbf{Iteration 1}} & \multicolumn{2}{c}{\textbf{Iteration 2}} & \multicolumn{2}{c}{\textbf{Iteration 3}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
& Success Rate & Build Rate & Success Rate & Build Rate & Success Rate & Build Rate \\
\midrule
DeepSeek-v3 & 6.61 & 44.26 & 15.09 & 77.57 & 16.98 & 79.44 \\
GPT-4-turbo & 5.79 & 40.16 & 10.96 & 60.81 & 8.16 & 56.00 \\
GPT-4o & 9.09 & 54.10 & 13.89 & 61.47 & 15.74 & 70.64 \\
GPT-4o-mini & 6.61 & 42.62 & 13.21 & 46.73 & 10.38 & 44.86 \\
Qwen-plus-1220 & 9.09 & 45.08 & 4.96 & 41.80 & 7.44 & 63.93 \\
Claude-3-5-sonnet-20240620 & 3.31 & 46.72 & 11.71 & 80.36 & 11.29 & 54.84 \\
\bottomrule
\end{tabular}
    % \begin{tablenotes}
    %     \footnotesize
    %     \item HN: Number of holes in program; Env Merge: Environment Merge; HB Merge: Hole Bindings Merge
    %     \item Parse Code refers to the ``Parser'' in Figure \ref{framework}; Forward Eval refers to the “Forward Evaluator” described in Section \ref{sec:feval}; Parse HTML refers to ``HTML Parser''; Backward Eval refers to ``Backward Evaluato'' described in Section \ref{sec:beval}; Print refers to ``Printer'' in Figure \ref{framework}.
    %   \end{tablenotes}
    % \end{threeparttable}
    \label{tab:overall-performance}
\end{table*}

==> figures/Performance02.tex <==
\begin{table*}[htb]
\caption{Build rates (\%) for different repositories across various models.}
\centering
\footnotesize
\begin{tabular}{lcccccc}
\toprule
\textbf{Repo} & GPT-4o & GPT-4o-mini & GPT-4-turbo & Qwen-plus & Claude-3.5 & DeepSeek-v3 \\
\midrule
promise & 44.4 & 44.4 & 0.0 & 44.4 & 100.0 & 44.4 \\
table-module & 76.2 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
double-buffer & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
decorator & 100.0 & 0.0 & 0.0 & 0.0 & 66.7 & 66.7 \\
producer-consumer & 0.0 & 10.0 & 33.3 & 33.3 & 33.3 & 100.0 \\
double-dispatch & 100.0 & 25.0 & 62.5 & 79.2 & 100.0 & 45.8 \\
partial-response & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
converter & 80.0 & 80.0 & 80.0 & 100.0 & 100.0 & 80.0 \\
caching & 100.0 & 50.0 & 50.0 & 100.0 & 50.0 & 50.0 \\
unit-of-work & 100.0 & 100.0 & 0.0 & 100.0 & 60.0 & 100.0 \\
game-loop & 22.2 & 2.2 & 88.9 & 100.0 & 100.0 & 100.0\\
type-object & 0.0 & 0.0 & 0.0 & 60.0 & 0.0 & 0.0 \\
bytecode & 9.1 & 18.2 & 18.2 & 9.1 & 100.0 & 100.0 \\
\bottomrule
\end{tabular}
\label{tab:build-rates}
\end{table*}

==> figures/Performance03.tex <==
% Unit Test Pass Rate Table
\begin{table*}[htb]
\caption{Unit test pass rates (\%) for different repositories across various models.}
\footnotesize
\centering
\begin{tabular}{lcccccc}
\toprule
\textbf{Repo} & GPT-4o & GPT-4o-mini & GPT-4-turbo & Qwen-plus & Claude-3.5 & DeepSeek-v3 \\
\midrule
promise & 22.2 & 11.1 & 0.0 & 11.1 & 11.1 & 11.1 \\
table-module & 4.8 & 9.5 & 9.5 & 9.5 & 9.5 & 9.5 \\
double-buffer & 42.9 & 42.9 & 42.9 & 42.9 & 42.9 & 42.9 \\
decorator & 33.3 & 0.0 & 0.0 & 0.0 & 33.3 & 0.0 \\
producer-consumer & 0.0 & 33.3 & 0.0 & 0.0 & 33.3 & 33.3 \\
double-dispatch & 45.8 & 16.7 & 12.5 & 12.5 & 16.7 & 8.3 \\
partial-response & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
converter & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
caching & 10.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
unit-of-work & 50.0 & 40.0 & 0.0 & 20.0 & 50.0 & 50.0 \\
game-loop & 0.0 & 22.2 & 11.1 & 11.1 & 11.1 & 33.3 \\
type-object & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
bytecode & 9.1 & 9.1 & 9.1 & 9.1 & 9.1 & 18.2 \\
\bottomrule
\end{tabular}
\label{tab:unit-test-pass-rates}
\end{table*}

==> sections/threats_to_validity.tex <==
\section{Threats to Validity}
